Towards a Golden Classifier-Free Guidance Path via Foresight Fixed Point Iterations

Classifier-Free Guidance (CFG) is an essential component of text-to-image diffusion models, and understanding and advancing its operational mechanisms remains a central focus of research. Existing approaches stem from divergent theoretical interpretations, thereby limiting the design space and obscuring key design choices. To address this, we propose a unified perspective that reframes conditional guidance as fixed point iterations, seeking to identify a golden path where latents produce consistent outputs under both conditional and unconditional generation. We demonstrate that CFG and its variants constitute a special case of single-step short-interval iteration, which is theoretically proven to exhibit inefficiency. To this end, we introduce Foresight Guidance (FSG), which prioritizes solving longer-interval subproblems in early diffusion stages with increased iterations. Extensive experiments across diverse datasets and model architectures validate the superiority of FSG over state-of-the-art methods in both image quality and computational efficiency. Our work offers novel perspectives for conditional guidance and unlocks the potential of adaptive design.

==> packages.tex <==
% Encoding and font
\usepackage[utf8]{inputenc}   % UTF-8 input encoding
\usepackage[T1]{fontenc}      % 8-bit T1 fonts
\usepackage{lmodern}          % Latin Modern font (optional but recommended)

% Math packages
\usepackage{amsmath, amsfonts, amssymb, amsthm} % Core math functionalities
\usepackage{bm}               % Bold math symbols
\usepackage{mathrsfs}         % Script fonts in math
\usepackage{bbold}            % Blackboard bold numbers
\usepackage{xfrac}            % Nice fractions (e.g. \sfrac)
\usepackage{nicefrac}         % Compact symbols for 1/2, etc.

% Document layout and spacing
%\usepackage{fullpage}         % Narrower margins than article default
\usepackage{setspace}         % Control line spacing
\usepackage{microtype}        % Microtypography improvements
\usepackage{enumitem}         % Customizable lists

% Graphics and figures
\usepackage{graphicx}         % Including images
\usepackage{float}            % Improved float control (e.g. [H])
\usepackage{subcaption}       % Subfigures and subcaptions
\usepackage{wrapfig}          % Wrapped figures
\usepackage{caption}          % Captions customization

% Tables
\usepackage{booktabs}         % Professional-quality tables
\usepackage{tabularx}         % Tables with adjustable width
\usepackage{multirow}         % Multirow cells in tables
\usepackage{makecell}         % More control over table cells

% Algorithms
\usepackage[ruled,vlined,linesnumbered]{algorithm2e} % Algorithm environment with line numbering

% Hyperlinks and URLs
\usepackage{hyperref}         % Hyperlinks support
\usepackage{url}              % URL formatting

% Colors and boxes
\usepackage{xcolor}           % Color support
\usepackage{tcolorbox}        % Colored/fancy boxes
\usepackage{framed}           % Framed boxes
\usepackage{ulem}             % Underlining / strikethrough (e.g. \sout)

% Citations
\usepackage{natbib}           % Flexible bibliography styles
\usepackage{cite}             % Numerical citations support

% Additional symbols
\usepackage{pifont}           % Dingbats symbols

% Clever referencing
\usepackage[nameinlink,capitalize]{cleveref} % Smart cross referencing

% Optional (commented out in your original)
% \usepackage{babel}          % Language and hyphenation rules (uncomment if needed)
